Particle-Based Shape Modeling for Arbitrary Regions-of-Interest

Statistical Shape Modeling (SSM) is a quantitative method for analyzing morphological variations in anatomical structures. These analyses often necessitate building models on targeted anatomical regions of interest to focus on specific morphological features. We propose an extension to \particle-based shape modeling (PSM), a widely used SSM framework, to allow shape modeling to arbitrary regions of interest. Existing methods to define regions of interest are computationally expensive and have topological limitations. To address these shortcomings, we use mesh fields to define free-form constraints, which allow for delimiting arbitrary regions of interest on shape surfaces. Furthermore, we add a quadratic penalty method to the model optimization to enable computationally efficient enforcement of any combination of cutting-plane and free-form constraints. We demonstrate the effectiveness of this method on a challenging synthetic dataset and two medical datasets.

==> problem_formulation.tex <==
\section{Problem Formulation}
\label{sec:problem_formulation}

\begin{itemize}
    \item \SE{notations}
    \item Briefly give context on the \SE{PSM} objective \SE{(discuss sampling and corresponding) -- should be brief but self-contained description of PSM.}
    \item The inequality constraints formulation.
\end{itemize}

\subsection{Unconstrained Optimization Problem}
Touch on how this can be turned into an unconstrained problem using augmented lagrangian methods.
